AndroVault: Constructing Knowledge Graph from Millions of Android Apps for Automated Analysis

Data driven research on Android has gained a great momentum these years. The abundance of data facilitates knowledge learning, however, also increases the difficulty of data preprocessing. Therefore, it is non-trivial to prepare a demanding and accurate set of data for research. In this work, we put forward AndroVault, a framework for the Android research composing of data collection, knowledge representation and knowledge extraction. It has started with a long-running web crawler for data collection (both apps and description) since 2013, which guarantees the timeliness of data; With static analysis and dynamic analysis of the collected data, we compute a variety of attributes to characterize Android apps. After that, we employ a knowledge graph to connect all these apps by computing their correlation in terms of attributes; Last, we leverage multiple technologies such as logical inference, machine learning, and correlation analysis to extract facts (more accurate and demanding, either high level or not, data) that are beneficial for a specific research problem. With the produced data of high quality, we have successfully conducted many research works including malware detection, code generation, and Android testing. We would like to release our data to the research community in an authenticated manner, and encourage them to conduct productive research.

==> datacol.tex <==
\section{Data Collection}

\subsection{App Crawler}

\subsection{Market}

\subsection{Statistics}



To characterize these Android apps, we figure out the following attributes for each app.
\begin{table}
  \centering
  \begin{tabular}{rl}
  \toprule
  \textbf{Entry} & \textbf{Description} \\ \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  SHA256 & a hash value for the whole apk file. \\
  Certificate& with which Android apps are digitally signed for integrity.\\
  Creation date& representing the date when the developer creates this app.\\
  Marketplace& from which market is the app downloaded.\\
  Package name& a Java-language-style name for apps, which serves as an identifier on Android.\\
  Version code& denoting the upgrade history of apps.\\
  Requested permission\\
  Sensitive APIs&\\
  Native code&\\
  Reflection&\\
  Contained files&\\
  Component&\\
  PHA family&\\
  Sensitive Strings&\\
  Dependent Libraries&\\
  \bottomrule
\end{tabular}
  \caption{Metainformation of Android apps}\label{tbl:metadata}
\end{table}

